Riemannian optimization for non-centered mixture of scaled Gaussian distributions

This paper studies the statistical model of the non-centered mixture of scaled Gaussian distributions (NC-MSG). Using the Fisher-Rao information geometry associated to this distribution, we derive a Riemannian gradient descent algorithm. This algorithm is leveraged for two minimization problems. The first one is the minimization of a regularized negative log-likelihood (NLL). The latter makes the trade-off between a white Gaussian distribution and the NC-MSG. Conditions on the regularization are given so that the existence of a minimum to this problem is guaranteed without assumptions on the samples. Then, the Kullback-Leibler (KL) divergence between two NC-MSG is derived. This divergence enables us to define a minimization problem to compute centers of mass of several NC-MSGs. The proposed Riemannian gradient descent algorithm is leveraged to solve this second minimization problem. Numerical experiments show the good performance and the speed of the Riemannian gradient descent on the two problems. Finally, a Nearest centroid classifier is implemented leveraging the KL divergence and its associated center of mass. Applied on the large scale dataset Breizhcrops, this classifier shows good accuracies as well as robustness to rigid transformations of the test set.

==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_16-10-52/AA_vs_mean_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={AA},
ymin=0.0912, ymax=0.5268,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.135
0.00083405026860003 0.135
0.00139127970110356 0.135
0.00232079441680639 0.136
0.00387131841340563 0.136
0.00645774832507442 0.138
0.0107721734501594 0.149
0.0179690683190231 0.151
0.029974212515947 0.152
0.05 0.165
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.146
0.00083405026860003 0.147
0.00139127970110356 0.148
0.00232079441680639 0.149
0.00387131841340563 0.149
0.00645774832507442 0.171
0.0107721734501594 0.118
0.0179690683190231 0.113
0.029974212515947 0.12
0.05 0.119
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.156
0.00083405026860003 0.156
0.00139127970110356 0.156
0.00232079441680639 0.156
0.00387131841340563 0.156
0.00645774832507442 0.155
0.0107721734501594 0.155
0.0179690683190231 0.156
0.029974212515947 0.156
0.05 0.148
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.507
0.00083405026860003 0.507
0.00139127970110356 0.505
0.00232079441680639 0.494
0.00387131841340563 0.449
0.00645774832507442 0.37
0.0107721734501594 0.242
0.0179690683190231 0.189
0.029974212515947 0.151
0.05 0.111
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.493
0.00083405026860003 0.49
0.00139127970110356 0.479
0.00232079441680639 0.475
0.00387131841340563 0.405
0.00645774832507442 0.298
0.0107721734501594 0.214
0.0179690683190231 0.187
0.029974212515947 0.183
0.05 0.149
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.477
0.00083405026860003 0.477
0.00139127970110356 0.477
0.00232079441680639 0.478
0.00387131841340563 0.476
0.00645774832507442 0.467
0.0107721734501594 0.417
0.0179690683190231 0.264
0.029974212515947 0.168
0.05 0.115
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_16-10-52/OA_vs_mean_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={OA},
ymin=-0.02145, ymax=0.58245,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.08
0.00083405026860003 0.08
0.00139127970110356 0.081
0.00232079441680639 0.081
0.00387131841340563 0.081
0.00645774832507442 0.081
0.0107721734501594 0.083
0.0179690683190231 0.085
0.029974212515947 0.088
0.05 0.096
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.155
0.00083405026860003 0.157
0.00139127970110356 0.159
0.00232079441680639 0.163
0.00387131841340563 0.169
0.00645774832507442 0.179
0.0107721734501594 0.193
0.0179690683190231 0.212
0.029974212515947 0.242
0.05 0.284
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.225
0.00083405026860003 0.225
0.00139127970110356 0.226
0.00232079441680639 0.225
0.00387131841340563 0.225
0.00645774832507442 0.225
0.0107721734501594 0.225
0.0179690683190231 0.223
0.029974212515947 0.215
0.05 0.186
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.549
0.00083405026860003 0.546
0.00139127970110356 0.538
0.00232079441680639 0.51
0.00387131841340563 0.429
0.00645774832507442 0.222
0.0107721734501594 0.034
0.0179690683190231 0.026
0.029974212515947 0.026
0.05 0.026
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.554
0.00083405026860003 0.547
0.00139127970110356 0.529
0.00232079441680639 0.486
0.00387131841340563 0.376
0.00645774832507442 0.169
0.0107721734501594 0.032
0.0179690683190231 0.021
0.029974212515947 0.019
0.05 0.021
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.555
0.00083405026860003 0.554
0.00139127970110356 0.551
0.00232079441680639 0.545
0.00387131841340563 0.532
0.00645774832507442 0.494
0.0107721734501594 0.377
0.0179690683190231 0.109
0.029974212515947 0.019
0.05 0.006
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_16-10-52/f1_weighted_vs_mean_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={f1\_weighted},
ymin=-0.0294, ymax=0.6394,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.1
0.00083405026860003 0.101
0.00139127970110356 0.101
0.00232079441680639 0.101
0.00387131841340563 0.102
0.00645774832507442 0.103
0.0107721734501594 0.106
0.0179690683190231 0.11
0.029974212515947 0.116
0.05 0.125
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.217
0.00083405026860003 0.219
0.00139127970110356 0.221
0.00232079441680639 0.225
0.00387131841340563 0.229
0.00645774832507442 0.235
0.0107721734501594 0.241
0.0179690683190231 0.236
0.029974212515947 0.224
0.05 0.213
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.233
0.00083405026860003 0.233
0.00139127970110356 0.233
0.00232079441680639 0.233
0.00387131841340563 0.232
0.00645774832507442 0.232
0.0107721734501594 0.232
0.0179690683190231 0.23
0.029974212515947 0.227
0.05 0.203
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.601
0.00083405026860003 0.599
0.00139127970110356 0.592
0.00232079441680639 0.57
0.00387131841340563 0.497
0.00645774832507442 0.277
0.0107721734501594 0.015
0.0179690683190231 0.002
0.029974212515947 0.002
0.05 0.001
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.609
0.00083405026860003 0.604
0.00139127970110356 0.59
0.00232079441680639 0.552
0.00387131841340563 0.44
0.00645774832507442 0.211
0.0107721734501594 0.025
0.0179690683190231 0.006
0.029974212515947 0.003
0.05 0.002
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.607
0.00083405026860003 0.606
0.00139127970110356 0.604
0.00232079441680639 0.6
0.00387131841340563 0.591
0.00645774832507442 0.562
0.0107721734501594 0.462
0.0179690683190231 0.147
0.029974212515947 0.01
0.05 0.002
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_16-10-52/kappa_vs_mean_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={kappa},
ymin=-0.02305, ymax=0.48405,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.031
0.00083405026860003 0.031
0.00139127970110356 0.031
0.00232079441680639 0.03
0.00387131841340563 0.031
0.00645774832507442 0.031
0.0107721734501594 0.031
0.0179690683190231 0.031
0.029974212515947 0.03
0.05 0.029
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.072
0.00083405026860003 0.073
0.00139127970110356 0.074
0.00232079441680639 0.076
0.00387131841340563 0.078
0.00645774832507442 0.081
0.0107721734501594 0.086
0.0179690683190231 0.088
0.029974212515947 0.088
0.05 0.077
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.099
0.00083405026860003 0.099
0.00139127970110356 0.099
0.00232079441680639 0.099
0.00387131841340563 0.098
0.00645774832507442 0.098
0.0107721734501594 0.098
0.0179690683190231 0.097
0.029974212515947 0.095
0.05 0.079
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.458
0.00083405026860003 0.455
0.00139127970110356 0.446
0.00232079441680639 0.419
0.00387131841340563 0.341
0.00645774832507442 0.164
0.0107721734501594 0.021
0.0179690683190231 0.01
0.029974212515947 0.004
0.05 0
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.461
0.00083405026860003 0.454
0.00139127970110356 0.436
0.00232079441680639 0.393
0.00387131841340563 0.288
0.00645774832507442 0.117
0.0107721734501594 0.024
0.0179690683190231 0.016
0.029974212515947 0.012
0.05 0.008
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.459
0.00083405026860003 0.457
0.00139127970110356 0.454
0.00232079441680639 0.449
0.00387131841340563 0.436
0.00645774832507442 0.399
0.0107721734501594 0.291
0.0179690683190231 0.076
0.029974212515947 0.013
0.05 0.001
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_20-28-43/AA_vs_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={AA},
ymin=0.06085, ymax=0.52615,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.135
0.00083405026860003 0.135
0.00139127970110356 0.135
0.00232079441680639 0.135
0.00387131841340563 0.135
0.00645774832507442 0.135
0.0107721734501594 0.135
0.0179690683190231 0.135
0.029974212515947 0.135
0.05 0.134
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.145
0.00083405026860003 0.145
0.00139127970110356 0.145
0.00232079441680639 0.145
0.00387131841340563 0.145
0.00645774832507442 0.145
0.0107721734501594 0.145
0.0179690683190231 0.145
0.029974212515947 0.144
0.05 0.144
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.156
0.00083405026860003 0.156
0.00139127970110356 0.157
0.00232079441680639 0.166
0.00387131841340563 0.165
0.00645774832507442 0.164
0.0107721734501594 0.159
0.0179690683190231 0.137
0.029974212515947 0.111
0.05 0.082
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.505
0.00083405026860003 0.503
0.00139127970110356 0.501
0.00232079441680639 0.49
0.00387131841340563 0.449
0.00645774832507442 0.371
0.0107721734501594 0.251
0.0179690683190231 0.19
0.029974212515947 0.165
0.05 0.13
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.496
0.00083405026860003 0.496
0.00139127970110356 0.482
0.00232079441680639 0.477
0.00387131841340563 0.463
0.00645774832507442 0.393
0.0107721734501594 0.304
0.0179690683190231 0.206
0.029974212515947 0.168
0.05 0.131
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.477
0.00083405026860003 0.478
0.00139127970110356 0.479
0.00232079441680639 0.479
0.00387131841340563 0.478
0.00645774832507442 0.468
0.0107721734501594 0.419
0.0179690683190231 0.331
0.029974212515947 0.244
0.05 0.182
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_20-28-43/OA_vs_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={OA},
ymin=-0.02095, ymax=0.59395,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.08
0.00083405026860003 0.08
0.00139127970110356 0.08
0.00232079441680639 0.08
0.00387131841340563 0.08
0.00645774832507442 0.08
0.0107721734501594 0.08
0.0179690683190231 0.08
0.029974212515947 0.08
0.05 0.081
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.153
0.00083405026860003 0.153
0.00139127970110356 0.153
0.00232079441680639 0.153
0.00387131841340563 0.153
0.00645774832507442 0.153
0.0107721734501594 0.154
0.0179690683190231 0.154
0.029974212515947 0.154
0.05 0.155
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.224
0.00083405026860003 0.223
0.00139127970110356 0.221
0.00232079441680639 0.218
0.00387131841340563 0.213
0.00645774832507442 0.204
0.0107721734501594 0.188
0.0179690683190231 0.156
0.029974212515947 0.11
0.05 0.07
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.552
0.00083405026860003 0.551
0.00139127970110356 0.547
0.00232079441680639 0.532
0.00387131841340563 0.472
0.00645774832507442 0.286
0.0107721734501594 0.067
0.0179690683190231 0.024
0.029974212515947 0.015
0.05 0.007
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.562
0.00083405026860003 0.562
0.00139127970110356 0.56
0.00232079441680639 0.55
0.00387131841340563 0.509
0.00645774832507442 0.362
0.0107721734501594 0.098
0.0179690683190231 0.027
0.029974212515947 0.016
0.05 0.007
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.559
0.00083405026860003 0.561
0.00139127970110356 0.563
0.00232079441680639 0.566
0.00387131841340563 0.565
0.00645774832507442 0.549
0.0107721734501594 0.49
0.0179690683190231 0.35
0.029974212515947 0.235
0.05 0.132
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_20-28-43/f1_weighted_vs_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={f1\_weighted},
ymin=-0.0254, ymax=0.6434,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.1
0.00083405026860003 0.1
0.00139127970110356 0.1
0.00232079441680639 0.1
0.00387131841340563 0.1
0.00645774832507442 0.1
0.0107721734501594 0.101
0.0179690683190231 0.101
0.029974212515947 0.102
0.05 0.103
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.215
0.00083405026860003 0.215
0.00139127970110356 0.215
0.00232079441680639 0.215
0.00387131841340563 0.215
0.00645774832507442 0.215
0.0107721734501594 0.215
0.0179690683190231 0.215
0.029974212515947 0.215
0.05 0.214
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.233
0.00083405026860003 0.232
0.00139127970110356 0.232
0.00232079441680639 0.231
0.00387131841340563 0.229
0.00645774832507442 0.224
0.0107721734501594 0.211
0.0179690683190231 0.179
0.029974212515947 0.115
0.05 0.06
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.602
0.00083405026860003 0.6
0.00139127970110356 0.595
0.00232079441680639 0.58
0.00387131841340563 0.527
0.00645774832507442 0.335
0.0107721734501594 0.052
0.0179690683190231 0.01
0.029974212515947 0.009
0.05 0.005
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.613
0.00083405026860003 0.613
0.00139127970110356 0.61
0.00232079441680639 0.6
0.00387131841340563 0.562
0.00645774832507442 0.415
0.0107721734501594 0.106
0.0179690683190231 0.015
0.029974212515947 0.01
0.05 0.006
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.61
0.00083405026860003 0.61
0.00139127970110356 0.611
0.00232079441680639 0.613
0.00387131841340563 0.61
0.00645774832507442 0.591
0.0107721734501594 0.52
0.0179690683190231 0.337
0.029974212515947 0.209
0.05 0.151
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-27_20-28-43/kappa_vs_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={kappa},
ymin=-0.01715, ymax=0.49215,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.031
0.00083405026860003 0.031
0.00139127970110356 0.031
0.00232079441680639 0.031
0.00387131841340563 0.031
0.00645774832507442 0.031
0.0107721734501594 0.031
0.0179690683190231 0.031
0.029974212515947 0.031
0.05 0.031
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.071
0.00083405026860003 0.071
0.00139127970110356 0.071
0.00232079441680639 0.071
0.00387131841340563 0.07
0.00645774832507442 0.07
0.0107721734501594 0.07
0.0179690683190231 0.07
0.029974212515947 0.07
0.05 0.069
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.099
0.00083405026860003 0.099
0.00139127970110356 0.098
0.00232079441680639 0.098
0.00387131841340563 0.096
0.00645774832507442 0.093
0.0107721734501594 0.085
0.0179690683190231 0.067
0.029974212515947 0.035
0.05 0.009
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.459
0.00083405026860003 0.458
0.00139127970110356 0.454
0.00232079441680639 0.437
0.00387131841340563 0.377
0.00645774832507442 0.209
0.0107721734501594 0.05
0.0179690683190231 0.021
0.029974212515947 0.014
0.05 0.006
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.468
0.00083405026860003 0.469
0.00139127970110356 0.465
0.00232079441680639 0.455
0.00387131841340563 0.412
0.00645774832507442 0.274
0.0107721734501594 0.074
0.0179690683190231 0.023
0.029974212515947 0.014
0.05 0.006
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.463
0.00083405026860003 0.464
0.00139127970110356 0.466
0.00232079441680639 0.468
0.00387131841340563 0.465
0.00645774832507442 0.446
0.0107721734501594 0.377
0.0179690683190231 0.229
0.029974212515947 0.13
0.05 0.063
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-28_00-46-19/AA_vs_mean_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={AA},
ymin=0.0556, ymax=0.5264,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.135
0.00083405026860003 0.135
0.00139127970110356 0.135
0.00232079441680639 0.135
0.00387131841340563 0.136
0.00645774832507442 0.137
0.0107721734501594 0.148
0.0179690683190231 0.15
0.029974212515947 0.151
0.05 0.163
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.146
0.00083405026860003 0.147
0.00139127970110356 0.148
0.00232079441680639 0.148
0.00387131841340563 0.149
0.00645774832507442 0.171
0.0107721734501594 0.118
0.0179690683190231 0.113
0.029974212515947 0.119
0.05 0.117
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.156
0.00083405026860003 0.156
0.00139127970110356 0.157
0.00232079441680639 0.157
0.00387131841340563 0.166
0.00645774832507442 0.164
0.0107721734501594 0.148
0.0179690683190231 0.136
0.029974212515947 0.105
0.05 0.077
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.505
0.00083405026860003 0.505
0.00139127970110356 0.501
0.00232079441680639 0.484
0.00387131841340563 0.422
0.00645774832507442 0.285
0.0107721734501594 0.185
0.0179690683190231 0.131
0.029974212515947 0.111
0.05 0.111
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.492
0.00083405026860003 0.49
0.00139127970110356 0.482
0.00232079441680639 0.468
0.00387131841340563 0.423
0.00645774832507442 0.34
0.0107721734501594 0.199
0.0179690683190231 0.134
0.029974212515947 0.111
0.05 0.111
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.478
0.00083405026860003 0.479
0.00139127970110356 0.48
0.00232079441680639 0.479
0.00387131841340563 0.474
0.00645774832507442 0.444
0.0107721734501594 0.348
0.0179690683190231 0.203
0.029974212515947 0.123
0.05 0.109
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-28_00-46-19/OA_vs_mean_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={OA},
ymin=-0.02055, ymax=0.58555,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.08
0.00083405026860003 0.081
0.00139127970110356 0.08
0.00232079441680639 0.081
0.00387131841340563 0.081
0.00645774832507442 0.082
0.0107721734501594 0.083
0.0179690683190231 0.085
0.029974212515947 0.087
0.05 0.095
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.155
0.00083405026860003 0.157
0.00139127970110356 0.159
0.00232079441680639 0.163
0.00387131841340563 0.169
0.00645774832507442 0.179
0.0107721734501594 0.193
0.0179690683190231 0.211
0.029974212515947 0.239
0.05 0.277
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.224
0.00083405026860003 0.223
0.00139127970110356 0.221
0.00232079441680639 0.219
0.00387131841340563 0.214
0.00645774832507442 0.204
0.0107721734501594 0.185
0.0179690683190231 0.148
0.029974212515947 0.096
0.05 0.07
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.551
0.00083405026860003 0.55
0.00139127970110356 0.542
0.00232079441680639 0.507
0.00387131841340563 0.38
0.00645774832507442 0.114
0.0107721734501594 0.027
0.0179690683190231 0.026
0.029974212515947 0.026
0.05 0.026
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.556
0.00083405026860003 0.55
0.00139127970110356 0.535
0.00232079441680639 0.493
0.00387131841340563 0.379
0.00645774832507442 0.17
0.0107721734501594 0.033
0.0179690683190231 0.027
0.029974212515947 0.026
0.05 0.026
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.558
0.00083405026860003 0.558
0.00139127970110356 0.557
0.00232079441680639 0.553
0.00387131841340563 0.539
0.00645774832507442 0.488
0.0107721734501594 0.316
0.0179690683190231 0.07
0.029974212515947 0.012
0.05 0.007
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-28_00-46-19/f1_weighted_vs_mean_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={f1\_weighted},
ymin=-0.0295, ymax=0.6415,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.101
0.00083405026860003 0.101
0.00139127970110356 0.101
0.00232079441680639 0.101
0.00387131841340563 0.102
0.00645774832507442 0.104
0.0107721734501594 0.106
0.0179690683190231 0.11
0.029974212515947 0.116
0.05 0.125
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.217
0.00083405026860003 0.219
0.00139127970110356 0.221
0.00232079441680639 0.225
0.00387131841340563 0.229
0.00645774832507442 0.235
0.0107721734501594 0.241
0.0179690683190231 0.237
0.029974212515947 0.224
0.05 0.213
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.233
0.00083405026860003 0.232
0.00139127970110356 0.232
0.00232079441680639 0.231
0.00387131841340563 0.228
0.00645774832507442 0.223
0.0107721734501594 0.208
0.0179690683190231 0.165
0.029974212515947 0.087
0.05 0.056
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.602
0.00083405026860003 0.6
0.00139127970110356 0.593
0.00232079441680639 0.564
0.00387131841340563 0.444
0.00645774832507442 0.139
0.0107721734501594 0.003
0.0179690683190231 0.002
0.029974212515947 0.001
0.05 0.001
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.611
0.00083405026860003 0.607
0.00139127970110356 0.596
0.00232079441680639 0.559
0.00387131841340563 0.44
0.00645774832507442 0.201
0.0107721734501594 0.009
0.0179690683190231 0.002
0.029974212515947 0.001
0.05 0.001
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.609
0.00083405026860003 0.609
0.00139127970110356 0.608
0.00232079441680639 0.605
0.00387131841340563 0.594
0.00645774832507442 0.552
0.0107721734501594 0.393
0.0179690683190231 0.097
0.029974212515947 0.013
0.05 0.005
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_acc_vs_affine_transfo_train_small_test_L1C/2022-06-28_00-46-19/kappa_vs_mean_rotation_transfo_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1.02)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={t},
xmin=0.000397164117362141, xmax=0.0629462705897084,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1},
xticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\)
},
y grid style={darkgray176},
ylabel={kappa},
ymin=-0.02315, ymax=0.48615,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0.0005 0.031
0.00083405026860003 0.031
0.00139127970110356 0.031
0.00232079441680639 0.031
0.00387131841340563 0.031
0.00645774832507442 0.031
0.0107721734501594 0.031
0.0179690683190231 0.031
0.029974212515947 0.03
0.05 0.029
};
\addlegendentry{Identity_Euclidean}
\addplot [semithick, darkorange25512714]
table {%
0.0005 0.072
0.00083405026860003 0.072
0.00139127970110356 0.074
0.00232079441680639 0.075
0.00387131841340563 0.078
0.00645774832507442 0.081
0.0107721734501594 0.086
0.0179690683190231 0.088
0.029974212515947 0.086
0.05 0.078
};
\addlegendentry{Mean_Vector_Euclidean}
\addplot [semithick, forestgreen4416044]
table {%
0.0005 0.099
0.00083405026860003 0.098
0.00139127970110356 0.098
0.00232079441680639 0.098
0.00387131841340563 0.096
0.00645774832507442 0.092
0.0107721734501594 0.083
0.0179690683190231 0.06
0.029974212515947 0.021
0.05 0.003
};
\addlegendentry{Covariance_Euclidean}
\addplot [semithick, crimson2143940]
table {%
0.0005 0.459
0.00083405026860003 0.457
0.00139127970110356 0.449
0.00232079441680639 0.414
0.00387131841340563 0.293
0.00645774832507442 0.08
0.0107721734501594 0.012
0.0179690683190231 0.005
0.029974212515947 0
0.05 0
};
\addlegendentry{Covariance_div_alpha_sym_0}
\addplot [semithick, mediumpurple148103189]
table {%
0.0005 0.463
0.00083405026860003 0.457
0.00139127970110356 0.442
0.00232079441680639 0.399
0.00387131841340563 0.292
0.00645774832507442 0.121
0.0107721734501594 0.016
0.0179690683190231 0.002
0.029974212515947 0
0.05 0
};
\addlegendentry{Location_covariance_div_alpha_sym_0}
\addplot [semithick, sienna1408675]
table {%
0.0005 0.461
0.00083405026860003 0.461
0.00139127970110356 0.46
0.00232079441680639 0.455
0.00387131841340563 0.44
0.00645774832507442 0.387
0.0107721734501594 0.23
0.0179690683190231 0.046
0.029974212515947 0.005
0.05 0.001
};
\addlegendentry{Location_covariance_texture_constrained_texture_div_alpha_sym_0_reg_L2_1e-11}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_tuning_train_val_small_L1C/2022-06-21_09-52-59/AA_alpha_sym_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=1.99526231496888e-21, xmax=5.01187233627272e-06,
xmode=log,
xtick style={color=black},
xtick={1e-23,1e-21,1e-19,1e-17,1e-15,1e-13,1e-11,1e-09,1e-07,1e-05,0.001},
xticklabels={
  \(\displaystyle {10^{-23}}\),
  \(\displaystyle {10^{-21}}\),
  \(\displaystyle {10^{-19}}\),
  \(\displaystyle {10^{-17}}\),
  \(\displaystyle {10^{-15}}\),
  \(\displaystyle {10^{-13}}\),
  \(\displaystyle {10^{-11}}\),
  \(\displaystyle {10^{-9}}\),
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-3}}\)
},
y grid style={darkgray176},
ymin=12.2, ymax=45.2,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=diamond*, mark size=3, mark options={solid}]
table {%
1e-20 16.9
3.59381366380464e-19 13.7
1.29154966501488e-17 31.9
4.64158883361279e-16 41
1.66810053720006e-14 42.4
5.99484250318942e-13 43
2.15443469003189e-11 43.7
7.74263682681128e-10 41.7
2.78255940220713e-08 37
1e-06 29.2
};
\addlegendentry{L2}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_tuning_train_val_small_L1C/2022-06-21_09-52-59/OA_alpha_sym_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=1.99526231496888e-21, xmax=5.01187233627272e-06,
xmode=log,
xtick style={color=black},
xtick={1e-23,1e-21,1e-19,1e-17,1e-15,1e-13,1e-11,1e-09,1e-07,1e-05,0.001},
xticklabels={
  \(\displaystyle {10^{-23}}\),
  \(\displaystyle {10^{-21}}\),
  \(\displaystyle {10^{-19}}\),
  \(\displaystyle {10^{-17}}\),
  \(\displaystyle {10^{-15}}\),
  \(\displaystyle {10^{-13}}\),
  \(\displaystyle {10^{-11}}\),
  \(\displaystyle {10^{-9}}\),
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-3}}\)
},
y grid style={darkgray176},
ymin=2.975, ymax=54.125,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=diamond*, mark size=3, mark options={solid}]
table {%
1e-20 5.3
3.59381366380464e-19 18.3
1.29154966501488e-17 41.5
4.64158883361279e-16 48.7
1.66810053720006e-14 50.1
5.99484250318942e-13 51.6
2.15443469003189e-11 51.8
7.74263682681128e-10 48.8
2.78255940220713e-08 42.9
1e-06 35.6
};
\addlegendentry{L2}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_tuning_train_val_small_L1C/2022-06-21_09-52-59/f1_weighted_alpha_sym_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=1.99526231496888e-21, xmax=5.01187233627272e-06,
xmode=log,
xtick style={color=black},
xtick={1e-23,1e-21,1e-19,1e-17,1e-15,1e-13,1e-11,1e-09,1e-07,1e-05,0.001},
xticklabels={
  \(\displaystyle {10^{-23}}\),
  \(\displaystyle {10^{-21}}\),
  \(\displaystyle {10^{-19}}\),
  \(\displaystyle {10^{-17}}\),
  \(\displaystyle {10^{-15}}\),
  \(\displaystyle {10^{-13}}\),
  \(\displaystyle {10^{-11}}\),
  \(\displaystyle {10^{-9}}\),
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-3}}\)
},
y grid style={darkgray176},
ymin=6.535, ymax=58.565,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=diamond*, mark size=3, mark options={solid}]
table {%
1e-20 8.9
3.59381366380464e-19 26.7
1.29154966501488e-17 47.8
4.64158883361279e-16 53.7
1.66810053720006e-14 54.5
5.99484250318942e-13 55.9
2.15443469003189e-11 56.2
7.74263682681128e-10 53.3
2.78255940220713e-08 46.7
1e-06 38
};
\addlegendentry{L2}
\end{axis}

\end{tikzpicture}


==> figures/classification/MDM_tuning_train_val_small_L1C/2022-06-21_09-52-59/kappa_alpha_sym_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=1.99526231496888e-21, xmax=5.01187233627272e-06,
xmode=log,
xtick style={color=black},
xtick={1e-23,1e-21,1e-19,1e-17,1e-15,1e-13,1e-11,1e-09,1e-07,1e-05,0.001},
xticklabels={
  \(\displaystyle {10^{-23}}\),
  \(\displaystyle {10^{-21}}\),
  \(\displaystyle {10^{-19}}\),
  \(\displaystyle {10^{-17}}\),
  \(\displaystyle {10^{-15}}\),
  \(\displaystyle {10^{-13}}\),
  \(\displaystyle {10^{-11}}\),
  \(\displaystyle {10^{-9}}\),
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-3}}\)
},
y grid style={darkgray176},
ymin=1.17, ymax=43.63,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, mark=diamond*, mark size=3, mark options={solid}]
table {%
1e-20 3.1
3.59381366380464e-19 11.9
1.29154966501488e-17 30.9
4.64158883361279e-16 38.5
1.66810053720006e-14 39.9
5.99484250318942e-13 41.5
2.15443469003189e-11 41.7
7.74263682681128e-10 38.3
2.78255940220713e-08 31.1
1e-06 22.4
};
\addlegendentry{L2}
\end{axis}

\end{tikzpicture}

